ANALYSE -- Learning to Attack Cyber-Physical Energy Systems With Intelligent Agents

The ongoing penetration of energy systems with information and communications technology (ICT) and the introduction of new markets increase the potential for malicious or profit-driven attacks that endanger system stability. To ensure security-of-supply, it is necessary to analyze such attacks and their underlying vulnerabilities, to develop countermeasures and improve system design. We propose ANALYSE, a machine-learning-based software suite to let learning agents autonomously find attacks in cyber-physical energy systems, consisting of the power system, ICT, and energy markets. ANALYSE is a modular, configurable, and self-documenting framework designed to find yet unknown attack types and to reproduce many known attack strategies in cyber-physical energy systems from the scientific literature.

==> Tooling paper for arxiv/acros.tex <==
\begin{acronym}[JSONP]\itemsep0pt
	\acro{DER}{distributed energy resource}
	\acro{DSO}{distribution system operator}
	\acro{PV}{photovoltaic}
	\acro{RES}{renewable energy resources}
	\acro{TSO}{transmission system operator}
	\acro{WT}{wind turbine}
	\acro{RL}{reinforcement learning}
    \acro{MAC}{media access control}
	\acro{DRL}{deep reinforcement learning}
	\acro{AI}{artificial intelligence}
	\acro{ICT}{information and communications technology}
	\acro{OPF}{optimal power flow}
	\acro{CPS}{cyber-physical system}
	\acrodefplural{CPS}[CPS]{cyber-physical systems}
	\acro{CPES}{cyber-physical energy system}
	\acrodefplural{CPES}[CPES]{cyber-physical energy systems}
	\acro{DoE}{design-of-experiments}
	\acro{ARL}{adversarial resilience learning}
    \acro{SIEM}{security information and event management}
    \acro{YAML}{YAML Ain't Markup Language}
\end{acronym}




==> Tooling paper for arxiv/commands.tex <==
\newcommand{\eg}{e.g.\xspace}
\newcommand{\ie}{i.e.\xspace}
\newcommand{\etal}{et al.\xspace}

\newcommand{\smasher}{ANALYSE\xspace}
\newcommand{\palaestrai}{palaestrAI\xspace}
\newcommand{\mosaik}{mosaik\xspace}
\newcommand{\arsenai}{arsenAI\xspace}
\newcommand{\midas}{MIDAS\xspace}

\newcommand{\lastaccess}{2022-10-07\xspace}

\newcommand{\elasticfootnote}{\footnote{\url{https://www.elastic.co/elastic-stack/}, last access \lastaccess}\xspace}
\newcommand{\rettijfootnote}{\footnote{\url{https://gitlab.com/frihsb/rettij/}, last access \lastaccess}\xspace}
\newcommand{\elkstackfootnote}{\footnote{\url{ https://www.elastic.co/de/elastic-stack/}, last access \lastaccess}\xspace}
\newcommand{\mosaikfootnote}{\footnote{\url{www.offis.mosaik.de}, last access: \lastaccess}\xspace}
\newcommand{\midasfootnote}{\footnote{\url{https://gitlab.com/midas-mosaik/midas}, last access: \lastaccess}\xspace}
\newcommand{\pandapowerfootnote}{\footnote{\url{https://pandapower.readthedocs.io}, last access: \lastaccess}\xspace}



==> Tooling paper for arxiv/conclusions.tex <==
\section{Conclusions}\label{sec:conclusion}
% TODO ThW
\smasher is a co-simulation-based tool-suite to use \ac{DRL} to find and analyze attack strategies in \aclp{CPES}. Its current version combines a power system, \ac{ICT}, and an energy market implementation. We designed \smasher to be modular, configurable, and self-documenting to allow for the investigation of diverse research questions. This way, \smasher is designed to reproduce a broad range of existing research and to find new attack strategies in interconnected multi-domain systems. 
\par 
Currently, \smasher focuses on a single learning attacker agent, but the long-term idea is to allow for multi-agent systems, add defender agents, analyze their interplay, and improve system design based on the findings. 
%\todo[inline]{Begrenzungen aufzeigen, z.B. bzgl. MAS and multi-agent-learning?}


% ThW: Macht gerne Vorschläge was hier reinkönnte (abgesehen von dem normalen Kram)

% ThW: Environment becomes more complex and slow (LFB, OPF etc) -> important research direction to speed up simulation. Otherwise RL will reach its limits

% Provide an extended framework for agents: Understand their actions (> XRL), provide safe learning, provide offline learning to incorporate domain knowledge, allow for online learning, provide a "deploy-and-forget" like approach where even parameters and hyperparameters shouldn't need to be tuned anymore.

==> Tooling paper for arxiv/impact.tex <==
\section{Impact}\label{sec:impact}

%\textbf{This is the main section of the article and the reviewers weight the description here appropriately}

The impact of \smasher can be derived directly from its features and the co-developed frameworks.
%Indicate in what way new research questions can be pursued as a result of the  software (if any).
% Physical attacks like [] are possible, market attacks like [wol21], false data injection like in [], etc. 
% Brings cross-domain attack research to next level! 
As mentioned before, most research in the field focuses on single domains and sub-systems. %, for example \cite{yan17} only on the power system or \cite{} on the \ac{ICT}. 
The coupling of power systems, markets, \ac{ICT}, and potentially other domains enables researchers to look at new research questions that focus on interconnected multi-domain systems and their interrelations. For example, \smasher has the potential to investigate research questions like "How much can profit on the energy market be increased when we apply false data injection at point xy in the system?" or "How much of the \ac{ICT} needs to be compromised by an attacker to create a blackout?". 
Normally, such research questions would require extensive implementation and modeling. With \smasher, the co-simulation only needs to be supplemented by the required simulators and models with little implementation effort, if they do not exist already.  
\par 
% See motivation: Intelligent (and/or learning) agents in multi-domain envs can be considered
Second, we can place learning agents at almost arbitrary places in the system. By defining their reward function as maximizing damage, we have a general tool to investigate potential attack strategies in \ac{CPES}. Similarly, it is possible to find market exploits by defining market profit as reward \cite{wol21}. 
However, the opposite is imaginable too. By defining the reward function as maximizing, \eg, system stability or welfare, we can determine possible defensive strategies like controller settings by learning them. Therefore, it is also possible to place attacker \textbf{and} defender agents into the system to investigate their interrelations, which is the \ac{ARL} approach \cite{fischer2018adversarial}. However, the  main focus of \smasher is the attack and vulnerability analysis.
% \todo[inline]{Sollten nicht auch Beispielergebnisse gezeigt werden?}
\par 
%Indicate in what way, and to what extent, the pursuit of existing research  questions is improved (if so).
% modular (easy to expand or change)
% A re-usable tool to research similar to [x, y, ...] -> not start from scratch -> examples of what could be done
% Easily place some learning agent in co-simulation and assign actuators/sensors (which is not easily possible!)
Besides enabling new research questions, \smasher will also prove helpful for existing research directions. Again, modularity and configurability are the key functionalities: 
For example, Wolgast \etal \cite{wol21} investigate attack scenarios in a coupled energy and reactive power market system. With \smasher, it would be possible to reproduce the research by removing the \ac{ICT} simulator and defining the \ac{RL} actuators, sensors, and reward according to the objective in the paper. Chen \etal \cite{che19b} apply false data injection attacks to attack automatic voltage control in the power network. Their work could be reproduced by removing the market simulation and again defining the \ac{RL} problem accordingly. 
In conclusion, \smasher builds a foundation to reproduce existing research in the field, investigate different variants of these scenarios, or increase their complexity.
\par 
%Indicate in what way the software has changed the daily practice of its users (if so).
\smasher is still newly published. However, we believe it can provide an important contribution to investigating unwanted attack scenarios in \ac{CPES} and to deriving potential countermeasures. 
%Indicate how widespread the use of the software is within and outside the intended user group.
\par 
%Indicate in what way the software is used in commercial settings and/or how it led to the creation of spin-off companies (if so).
% Maybe long term vision: Penetration testing of power system as a service?!
% For now, \smasher is  used purely for research and educational purposes. However, a potential long-term commercial usage could be penetration testing of power systems, \ac{ICT}, and energy markets as-a-service for their respective operators or regulators. 


% TODO? What is the impact for RL? Is a modular co-simulation as environment a contribution??? Does not really fit the focus of our work...


==> Tooling paper for arxiv/intro.tex <==

\section{Motivation and Significance}
%Introduce the scientific background and the motivation for developing the software.
%Explain why the software is important and describe the exact (scientific) 
%problem(s) it solves.
%Indicate in what way the software has contributed (or how it will contribute 
%in the future) to the process of scientific discovery; if available, this is to 
%be supported by citing a research paper using the software.
%Provide a description of the experimental setting (how does the user use the software?).
%Introduce related work in literature (cite or list algorithms used, other 
%software etc.).

%% Motivation/Background/Problem
% Increasing complexity of cyber-physical energy systems -> potential weaknesse
% More and more automation and intelligence in the system
Energy systems worldwide are evolving into increasingly complex systems due to an increasing amount of \acf{ICT} added for monitoring and controlling, as well as the inclusion of energy markets. This results in faster time scales, smart controllable loads, and more automation and intelligence in the system. Despite the intended effects of controllability, adaptability, and cost efficiency of these digitalized systems, the resulting \acfp{CPES} exhibit new challenges for system operators with their increased complexity \cite{7980942}.
% At the same time, high pressure to lower costs -> less robustness
While system complexity increases, grid operators are under increasing economic pressure to maintain grid stability at minimal costs and investments. It must be ensured that no shortcuts are taken in terms of robustness.
\par 
Meanwhile, energy systems increasingly become targets for cyber attacks, terrorism, warfare, and other unwanted interventions from adversarial players. Recent examples are the ongoing attacks on the Ukrainian power system since 2017 and on the Nordstream gas pipelines in 2022.
%For example, the cyber attacks on the Ukrainian power grid in December 2015 \cite{ei16} revealed such attack vectors. % (mehr Beispiele? z. B. https://www.golem.de/news/ukraine-krieg-russische-hacker-hatten-zugriff-auf-das-deutsche-stromnetz-2207-167248.html).
Primarily due to the increasing complexity and interleaving of these interconnected systems, we expect an increasing potential for such attacks \cite{vei20}, with potentially catastrophic consequences. Besides attacks with malicious intentions, another possible motivation is to maximize profit by exploiting the flawed design of energy markets \cite{wol21}. However, the potential consequences can be the same, i.e., destabilizing interconnected energy systems.
\par 
% Kurze Beschreibung / Absatz der drei Inseln von Markt, physischem Stromnetz und der IKT. Jede hat Regulierungen, aber übergreifende Auswirkungen können bisher kaum oder nur sehr langwierig betrachtet und als solche identifiziert werden (siehe Beinahe Blackout Sommer 2019 in DE)
\par

% problems: How to find unknown (!) weaknesses; explicit models are required 
Therefore, an important research task is to develop methodologies and tools to identify systemic vulnerabilities, potential attack vectors, and unwanted destabilization incentives in existing and future \acp{CPES}. This way, preventive measures can be taken to remove vulnerabilities or to deploy countermeasures.
One major issue is that the still unknown attack vectors are the most relevant ones because no defense mechanism exists for them, similar to zero-day attacks in cyber security. While a growing body of literature investigates attacks on power systems, mainly rather predictable attacks or variants of known strategies are considered. 
% Maybe related work better here instead of extra section?!
% For example, TODO here literature?!
However, given the systems-of-systems characteristics of \acp{CPES}, future attacks can exploit the system's increasing complexity and interleaving, making them impossible to foresee at design time with traditional approaches. 
\par 
% Intelligence in cyber physical energy systems / critical infrastructure
% -> investigate: Attacks (terrorism/warfare), manipulation (profit-driven), or simply systemic weaknesses
One emerging approach to search for unknown attack possibilities is to place learning \textit{attacker} agents within the system, \eg \cite{wol21, ni18, yan17}. In literature, mostly \ac{DRL} agents are trained to maximize damage in the system, for example, by creating a blackout \cite{ni18}. In \ac{RL}, an agent uses trial-and-error to find actions in an environment that maximize a reward function \cite{sut18}. Consequently, learning attacker agents will autonomously develop strategies to attack the system if such strategies are possible and rewarded during training. From a research perspective, this allows us to extract new and unknown attack vectors and to stress-test a given \ac{CPES} in simulation. This is a prerequisite to developing defensive strategies in the future.
% Current scenarios are too simple, because build for human researchers
However, the learning agent can only utilize the degrees of freedom and information given. This is especially relevant in research, where often over-simplified scenarios are considered.
For example,  in current research, the different layers of a \ac{CPES}, \ie, physical component layer, \ac{ICT} layer, and function layer are typically modeled and evaluated separately. However, a too-limited action space may restrict the agent's ability to find new strategies, resulting in a false sense of security if no attack possibilities are found.
% \todo[inline]{Hier frage ich mich, ob man nicht auf die Notwendigkeit von Co-Simulation mit entspr. Referenz hier direkt eingehen sollte.}
\par 
An \acl{AI} does not necessarily require a simplified system. Especially \ac{DRL} algorithms demonstrated how they can handle highly complex tasks, \eg, mastering the game of Go \cite{silver2016mastering}. 
% \todo[inline]{Solltem an wirklich Go anführen? Wir reden ja über complexity über Kopplung nicht-linearer Systeme, das ist eine andere Kategorie.}
Therefore, one next step in this research area is to move from simplified scenarios to more realistic and interconnected ones, yielding more realistic attack strategies. 
Applied to the energy system, \ac{ICT}, energy grids, and markets should be investigated more holistically as a \ac{CPES} to consider interdependencies.
\par 
%% Contributions (experimental setting)
In the following, we present \smasher (ANAlyzing compLex cYber-physical Systems wEaknesses), a tool-suite to analyze coupled power grids, \ac{ICT}, and market systems with learning agents for vulnerabilities and potential attack strategies. The main features of this software artifact are as follows:
% First co-simulation of energy system, energy market and ICT yet (is this true?)
% Place (potenitally multiple) learning agents in all domains and give them arbitrary sensors/actors/rewards
% Co-Simuluation allows for modularity -> easily expandable
\begin{itemize}
	\item \smasher is the first open-source tool-suite that combines power grid, energy market, and \ac{ICT} infrastructure into one coupled simulation to analyze them regarding vulnerabilities.
	
	% (Anmerkung ToW: Soweit ich das sehe ist gerade die Simulation der Energienetzdaten per MIDAS ja relativ ausgeklügelt mit dem Inbetrachtziehen der Wetterdaten etc.; haben die Agenten darauf eigentlich Zugriff und können sich bspw. anhand der Wettervorhersagen Strategien ausdenken? Auf jeden Fall sollte irgendwo genauer beschrieben werden, wie mehr oder weniger sophisticated die Einzelsimulatoren jeweils sind, denn so wie es hier aktuell steht, kann das ja alles oder nichts sein - auch ne IKT-Netz-Simulation kann man ja quasi komplett wegabstrahieren und trotzdem behaupten, dass man sie hat, dasselbe gilt für Energienetz- und sicher auch Marktsimulation) 
	\item It allows to place one or multiple learning (or non-learning) agents into the system that have access to sensors and actuators in all three domains. 
	\item \smasher is modular, configurable, self-documenting, and provides advanced data logging. 
\end{itemize}
% \todo[inline]{An irgendeiner Stelle ist die Reduktion auf Agenten, aber nicht Multi-Agenten wichtig - ich wäre als Leserin enttäuscht, wenn das zu spät käme. Insbesondere der Marktbezug lässt denken, das könnte das implizieren.}
Since \smasher utilizes a co-simulation framework, it is easily expandable, for example if alternative or additional domains need to be considered. % ThW TODO: Das besser in die Liste verschieben?
% Allows to re-produce attacks from literature
This way, \smasher is designed to reproduce known attack strategies and scenarios from literature or to find novel more complex attack vectors over multiple domains.
\par 
%% Structure
In section~\ref{sec:description}, we provide an overview of \smasher and its components. Further, we present its key functionalities. In section~\ref{sec:example}, we provide a short illustrative example how the tool-suite works. In section~\ref{sec:impact}, we discuss the potential impact of \smasher before we conclude our work with section \ref{sec:conclusion}. 

% \section{Related Work (1/2 page)}
% TODO: related work komplett in Intro unterbringen! Welche paper sind für attacks relevant und erwähnenswert?!

% DRL to investigate attacks as general topic,
% in ICT (eg false data injection),
% physical attacks,
% market attacks 
% Conclusion: All these papers use their own implementation -> almost no 
%open-source code, no comparability, always re-implementation required, 



==> Tooling paper for arxiv/software.tex <==
\section{Software Description: \smasher}\label{sec:description}
%Describe the software in as much as is necessary to establish a vocabulary 
%needed to explain its impact. 

% Not a single monolith -> multiple frameworks and modular simulators that work together -> smasher = interplay of everything to solve attack stuff
\smasher describes the concept of multiple frameworks and modular simulators that work together as a tool-suite to analyze agent misbehavior in \ac{CPES}. 
% Highly modular (mosaik)
% Lots of open-source tools re-used
% Each part can be used for own stuff (but were mainly developed for smasher!)
We have developed multiple open-source tools that fulfill different sub-tasks towards that general goal but can also be used independently. This way, we achieve the best possible re-usability of the different software parts and a highly modular software architecture.
In the following, we will present the interplay of the \smasher components, the details of each component, and the overall functionalities. 

\subsection{Software Architecture}
\begin{figure}[p]
    \centering
    \includegraphics[width=0.9\linewidth]{System-Components-crop.pdf}
    \caption{\smasher: interplay of system components.}
    \label{fig:system-components}
\end{figure}
% Storyline of the figure:
The architecture and interplay of \smasher and its components are shown in Figure~\ref{fig:system-components}, which we describe in the following section from top to bottom.
% We want to analyse some attack scenario (=scenario file/definition)
The goal is to analyze attack scenarios in \ac{CPES}. The \emph{scenarios} are defined in a declarative way by YAML\footnote{\url{https://yaml.org/}, last access: 2022-12-22} files and are the starting points of \smasher experiments. They define which power grid to use, how many agents act in that environment, their objectives, etc.
% From that we derifed software development
% From these scenarios on, we derived our software development.
% arsenai: Design of experiments -> starts palaestrai
The first step for an experiment is \arsenai, which translates the scenario file into multiple experiment runs by applying techniques from \ac{DoE}.
%palaestrai: RL framework: Train n agents in an environment
The experiment runs are performed by \palaestrai, an \ac{RL} framework that allows the training of one or multiple agents in an \ac{RL} environment.
% RL-Environment = midas/mosak co-simulation
To build modular \ac{RL} environments, we developed \midas, which assembles a single environment from multiple simulators -- in this case, power system simulator, market simulator, and \ac{ICT} simulator -- by using the co-simulation framework \mosaik.  
%\todo[inline]{Eigentschön wäre es, wenn Fig. 1 noch mal vorher als völlig vereinfachte Komponentensicht dargestellt würde, also nur die FUnktion in den Kästen. Das würde den Text hier sehr einfach verständlich machen.}
% Simulators
% All data into data base -> analyse final results
During the whole simulation and training, all relevant data is logged into a database. These data can later be analyzed regarding system vulnerabilities, noteworthy emerging agent strategies, potential countermeasures, etc.
The different components will be presented in more detail in the following sections. 

%SoftwareX: Give a short overview of the overall software architecture; provide a pictorial 
%component overview or similar (if possible). If necessary provide implementation details.




 
\subsubsection{Mosaik and MIDAS}

The open-source co-simulation framework mosaik\mosaikfootnote is, on a technical level, responsible for data exchange and synchronization of the different simulators \cite{steinbrink2019cpes}.
Mosaik follows a concept of so-called simulators and models.
A model can be anything, from a simple function to a complex simulation environment, while a simulator implements the mosaik API for that model.
A simulator can manage several models.
To allow different models to exchange data, they must be connected via mosaik.
The synchronization is done using individual but fixed time intervals for each simulator.

The more simulators and models are involved, the more complex the orchestration process of starting and connecting models and managing data flows becomes.
Therefore, we developed the open-source framework \midas\midasfootnote, which handles the assembly of mosaik scenarios and comes with some pre-configured smart grid simulators and scenarios. 
\midas also enables aggregating all mosaik simulators into an environment for \ac{RL} agents, defining actions, observations, and rewards.
% ThW gestrichen: \midas is controlled with configuration files, which allow for easy re-configuration of existing scenarios.

\subsubsection{Power System Simulator}
\smasher uses the power grid simulator pandapower\pandapowerfootnote  to simulate a power grid with its topology and power flows \cite{thurner2018pandapower}.
To achieve more realistic behavior, we also added simulators for publicly available load profiles and a simulator for a \ac{PV} model that takes real weather data as input.
Since the \ac{PV} models depend on environmental conditions, we added a simulator for publicly
available weather data as well.
Although all those simulators are individual components of the mosaik scenario, we comprise them as the power system simulator in the following for simplicity.


\subsubsection{Reactive Power Market Simulator}
% TODO: ThW
% Local power system -> wholesale market does not make sense -> local ancillary service market for reactive power for voltage control
As a market system, we added a local reactive power market: In this type of markets, the grid operator procures reactive power from generators and other energy resources in the local system, mainly to perform voltage control \cite{wol22}. 
% Cite my review paper  (susceptible to market power and manipulation) + cite market attack paper -> qmarkets were shown to be susceptible to attacks
Reactive power markets are still under active research and were shown to be susceptible to profit-oriented attacks \cite{wol21, buc21} and the exercise of market power \cite{wol22, zho02}. We chose to consider a reactive power market because their local nature allows having clear system boundaries, in contrast to, \eg, the wholesale energy market \cite{wol21}.
\par 
% However, most reactive markets are OPF-based -> terrible for RL environment 
Most reactive power market models from literature are based on solving an \ac{OPF}, \ie, the grid operator solves an optimization problem to determine the optimal reactive power procurement \cite{wol22}. That is problematic for \ac{DRL} since often thousands and millions of iterations are required.  
% Describe my market: Sensitivity (typical in voltage control) based, merit order + prices = most effective trade for minimal costshttps://www.overleaf.com/project/62e7dd910d02951a3073f8a3
To reduce computational effort, we implemented a non-\ac{OPF}-based market, where the grid operator accepts the cheapest and most useful reactive power offers to perform voltage control in the system. 
% The grid operator knows the price $p_Q$ and offered amount $dQ$ of each reactive power provider, the voltage values $U$ in the whole system, and the reactive power sensitivity $S=dU/dQ$, \ie the expected voltage change when reactive power is provided. In the case of a voltage violation (overvoltage/undervoltage), the grid operator can sort all offers regarding $S/p$, \ie biggest impact for smallest price, and accept the best offers until the voltage violation is cleared. 
% % This way limited in its capabilities, but still effective for voltage control (but nothing else like line load or loss min)
% Since the sensitivity $S$ is only a linear approximation, this procedure has some error compared to the \ac{OPF}, but is less computational expensive. 
\par 
To achieve competition, we also implemented some basic non-learning agents participating in the market. 
%
% (Maybe include this in MIDAS and describe together with MIDAS)
%
\subsubsection{rettij \ac{ICT} Simulator} 
The rettij\rettijfootnote \ac{ICT} simulator has been developed to support \ac{CPES} research regarding \ac{ICT} security \cite{Niehaus2022}. It provides a simple-to-use yet scalable network simulator that can be combined with co-simulation frameworks like mosaik. 
rettij makes use of the Linux network stack, as rettij's network components (i.e., switch, router, hosts) are based on containerization technology and use Kubernetes as an orchestrator. The network simulator's architecture allows to simulate realistic network traffic without the noise of management traffic that often occurs in plain container communication. rettij does not aim to simulate certain network technologies such as cellular or WiFi but chooses a more general approach where a normal \ac{MAC}-layer is simulated. However, the network channels can be throttled and delays and packet losses can be introduced to mimic such communication technologies. Network topologies are defined declaratively by YAML configuration files. It is possible to use any custom components within the simulation as long as it can run in a docker container. For \smasher, we implemented interfaces that allow for interaction between rettij and the agents to control and monitor parts of the network infrastructure. Sensors provide the ability to read network states, such as the utilization of network interfaces, while actuators offer the possibility to manipulate data in the network or restart targeted nodes. 
A more in-depth description of rettij and a standalone version of a co-simulation usage example can be found in \cite{Niehaus2022, AALE2020}.

% Zunahme von IT-Angriffen auf kritische Infrastruktur (Quelle: BSI-Lagebericht?)
% Bedarf, IT-Angriffe in komplexen infrastrukturen auf Daten und Beobachtungsbasis zu erkennen, steigt. 
% rettij Topics:
%\begin{itemize}
  %  \item  rettij simplicity to use by creating custom software in ao typical on how software today is delivered: containers
   % \item configuration files to be human readable
  %  \item list rettij features
  %  \item for smasher, focus on interfaces with mosaik and midas
  %  \item smasher: development of custom component, that is able to transfer data between the containers on the ethernet link
 %   \item providing sensors and actuator for the interaction with an agent
  %  \item outlook: integrate simulation components (such as midas nodes) into rettij-compatible container
%\end{itemize}




% first version has been published in \cite{AALE2020}
% further development and usage for projets has been presented in \cite{Niehaus2022}



% TODO: BFr and/or TWo

\subsubsection{\palaestrai: Learning Agents Framework}
% TODO: NWe and/or EVe

\palaestrai is a framework to train and evaluate learning agent systems. The difference to existing \ac{DRL} frameworks is its clear separation of agents, environment, and experimental framework. \palaestrai focuses on a reliable execution of experiments with learning agents in complex environments, including co-simulations. It allows the implementation of various learning agents (\ac{DRL}, neuroevolution, etc.) and a variety of environments. 

%Experiment documents define a proper plan for experimentation, including definition of parameters and factors of agent algorithms, environments, the definition of training and test phases, stopping conditions, etc.
The \palaestrai subpackage \emph{arsenAI} parses experiment documents and uses statistical means to generate several experiment run definitions with specific parameter combinations defined in the experiment document.
%The \emph{arsenAI} software package of \palaestrai's ecosystem uses these documents, which are written in YAML format, to sample the space created by the factors, creating experiment run documents from them. 
Each experiment run is reproducible; feeding the same experiment run document to different \palaestrai instances will produce the same experimentation result each time, which helps countering the AI reproducibility crisis \cite{hutson2018artificial,gundersen2018reproducible,haibe2020transparency}.
% The Agent consists of a Brain for learning and a Muscle for interacting with the environment (inference). %The Environment contains the simulation environment or serves as an interface to the environment with which the agent interacts. 
% \todo[inline]{Das Brain-Muscle-Konzept sollte noch etwas genauer ausgeführt werden, oder aber hier raus.}
The key design goal of \palaestrai was to facilitate complex experiments, where agents can act in different, co-simulated simulators that form an \ac{RL} environment while learning from the experiences gathered from all simulators. 


%\subsubsection{\arsenai: Desing of Experiments}
%In experiments, systems are investigated.
%Those systems may have numerous variable influences, some of which may be changed by the experimenter (factors), while others are fixed (parameters).
%Common goals of experiments are to examine an optimal combination of factors for the given system or to find out the influence of certain factors.
%Depending on the number of factors and their value ranges, the number of possible combinations increases rapidly.
%To acquire as much information as possible with as few experiment runs as possible, proper sampling strategies are required.
%In \palaestrai, experiment documents contain the definitions of agent and environment, including parameters and factor variations, interfaces in form of sensors and actuators, and the experiment schedule, \ie, define training and test phases as well as which combination of agents, environments, sensors, and actuators should be used.
%The \emph{arsenAI} software packages provides the necessary algorithms to select useful factor combinations across different experiment run phases and, if required, limits the number of run definitions generated.
%Those run definitions can be executed by the scheduler and the results of all those runs allow to perform statistical analysis.

\subsection{Software Functionalities}\label{sec:functionalities}
%Present the major functionalities of the software.
% \todo[inline]{Ich nehme an, dass die Struktur so vorgegeben ist, dass erst die Architektur und dann die functionalities kommen, oder? Ist etwas unintuitiv für mich. ThW: Ja, das ist leider so vorgegeben...}
% Configurable: Modular simulators, assignment of sensors/actuators, experiment run files, etc

The core of \smasher is the co-simulation ability gained from the mosaik interface. It interfaces to separate simulators for power grid, market, and \ac{ICT}. Through \palaestrai's approach, these three simulators can be treated as one large \ac{RL} environment. For example, an agent can observe the power grid's current state and decide to bid on the market based on this observation. The bid is then communicated to the market by \ac{ICT} components. The goal is to simulate potential attack vectors for analysis, such as manipulating the power grid through malicious assets, shutting an actor out of the market with denial-of-service attacks (DoS), or gaming the market through an agent that controls multiple assets. More importantly, \smasher allows learning agents to discover weaknesses that emerge through the interconnection of three complex systems.

To investigate and analyze a variety of potential attack scenarios, we emphasize the following key features:

\paragraph{Co-Simulation and Modularity} 
% Co-simulation as RL environment (nicht als Erste: http://www.ibpsa.org/proceedings/BSO2020/BSOV2020_Amrani.pdf)
% modular - exchange/add/remove simulators
\smasher uses \mosaik to aggregate multiple independently developed simulators to create a single \ac{RL} environment. This results in a modular tool where simulators can be added, removed, or exchanged easily. For example, a simulator of the gas system or the balancing power market could be added.

\paragraph{Self-Documentation with Run Files}
Inherited from \palaestrai, experiments in \smasher are defined with run files. Run files are YAML files that define which \ac{RL} algorithm, environment, actuators, sensors, objectives, etc. are used for the experiment. This improves documentation of large-scale experimentation because the exact experiment definition for every experiment is always automatically stored. 
% Place one or multiple agents
% Experiment definition
% Assign sensors/actuators arbitrarily (in contrast to for example gym, where an env is fix -> we can investigate diverse variants of the same env!!! env design important part that is neglected in applied RL)
Further, this allows us to investigate diverse variants of one environment. Usually, in \ac{RL} research, the environment is a fixed benchmark environment. However, in applied \ac{RL},  we often want to investigate multiple variants of the environment, \eg, to explore the consequences of different design decisions, like controller design, market design, etc.

\paragraph{Logging and Evaluation}
% Logging - evaluate experiments
To evaluate experiments, we designed a custom vulnerability-analyzer component. Its core concept stems from cyber-security, where log data from different sources is collected, harmonized, and shipped to a \ac{SIEM}. The \ac{SIEM} allows analyzing the data and correlations of events. To easier collect logs, the \smasher components create event logs and simulation status logs. Those logs are shipped to an Elasticsearch database and can be visualized with Elastic's Kibana interface. This typical Elastic stack\elkstackfootnote architecture allows efficient thread hunting \cite{elk-threat-hunting} for \ac{ICT}-security and is here used to approach experiment evaluation analysis. This flexible tool chain enables integrating more data towards a big data platform to detect interdependent attacks.
%\todo[inline]{Letzter Punkt: Was ist mit Experimental-Design? Ich nehme an, dass Ihr es nicht aufführt, weil es nicht SMASHER, sondern palestrAI ist?}

% \subsection{Sample code snippets analysis (optional)}
% ThW: I propose to not fill this optional section
% Why not discuss an Experiment Run definition here?
% ThW: If we have the space left, that would make sense :)
